Efficient GNN Explanation via Learning Removal-based Attribution

As Graph Neural Networks (GNNs) have been widely used in real-world applications, model explanations are required not only by users but also by legal regulations. However, simultaneously achieving high fidelity and low computational costs in generating explanations has been a challenge for current methods. In this work, we propose a framework of GNN explanation named LeArn Removal-based Attribution (LARA) to address this problem. Specifically, we introduce removal-based attribution and demonstrate its substantiated link to interpretability fidelity theoretically and experimentally. The explainer in LARA learns to generate removal-based attribution which enables providing explanations with high fidelity. A strategy of subgraph sampling is designed in LARA to improve the scalability of the training process. In the deployment, LARA can efficiently generate the explanation through a feed-forward pass. We benchmark our approach with other state-of-the-art GNN explanation methods on six datasets. Results highlight the effectiveness of our framework regarding both efficiency and fidelity. In particular, LARA is 3.5 times faster and achieves higher fidelity than the state-of-the-art method on the large dataset ogbn-arxiv (more than 160K nodes and 1M edges), showing its great potential in real-world applications. Our source code is available at https://anonymous.4open.science/r/LARA-10D8/README.md.

==> text/6-related-work.tex <==
\section{Related Work}
\subsection{GNN Explanations}
The model explanation is one of the emerging technologies in recent years due to the wide application of machine learning models, where a handful of explanation methods are proposed specifically for GNNs. 
Popular existing works can be divided into gradient-based, surrogate-based, decomposition-based and perturbation-based methods~\cite{yuan2022explainability, wang2022accelerating}. Gradient-based explanations follow a similar procedure as on image and text data. For instance, \citet{pope2019explainability} proposed CAM and GradCAM for graphs, which make use of the final fully-connected layer in the graph model to produce the feature map for nodes. 
% Surrogate-based methods employ an interpretable model to approximate the original msodel's behavior and use the explanations of the surrogate model;
Surrogate-based methods explain the original model via approximating it using an interpretable model~\cite{vu2020pgm,huang2022graphlime,zhang2021relex}. For example, the feature weights given by the algorithm Hilbert-Schmidt Independence Criterion Lasso \cite{yamada2014high} are used as explanations for the original GNN in \cite{huang2022graphlime}. Decomposition-based methods back-propagate the prediction score layer by layer into the input space following the designed decomposition
rules~\cite{feng2021degree,pope2019explainability,schnake2021higher}, while perturbation-based explanations assign importance scores to nodes or edges by observing output changes when masking different input features~\cite{ying2019gnnexplainer,luo2020parameterized,funke2020hard,yuan2021explainability}. 
Among these works, PGExplainer~\cite{luo2020parameterized} and GNNExplainer learn masks of edges by maximizing the mutual information between the predictions with and without masking.
Fewer efforts have been paid to real-time GNN explanations, and our project aims at providing faithful explanations for GNNs in an efficient manner.
%while decomposition-based methods distribute prediction into different layers or neurons following decomposition rules~\cite{feng2021degree,pope2019explainability,schnake2021higher}. 

\subsection{Amortized Explanations}
In amortized explanation methods, a learned explainer generates explanations for a batch of instances via a forward pass~\cite{covert2021explaining}. \cite{chuang2022cortx,jethani2021fastshap,chen2018learning,jethani2021have} showcased real-time explanations on image and tabular data. To be concrete, FastSHAP~\cite{jethani2021fastshap} 
proposed an objective function for an explainer to capture Shapley value distribution, achieving real-time explanations. CoRTX~\cite{chuang2022cortx} trained an explainer using positive and negative samples by minimizing the constrastive loss. Moreover, very few labels (ground truth explanations) were used during training to boost the interpretation performance.
% Amortized explanations include two core elements: an explainer model and an optimization function to train it. 
\citet{chen2018learning} realized an explainer returning a distribution over selected features given the input instance. The explainer was trained by maximizing the variational approximation of mutual information between selected features and the response variable from the target model. 
\citet{jethani2021have} proposed to train a global selector and predictor jointly, where the selector (REAL-X) identified the minimal subset of features to maximize the fidelity evaluated by a predictor model (EVAL-X).
Compared to previous amortized explanations, our explainer has no constraints of input shape (unlike image or tabular data) and adapts to irregular data (graph data). Furthermore, our proposed objective function is designed to enable high-fidelity explanation generation.  
